Towards Accurate Localization by Instance Search

Visual object localization is the key step in a series of object detection tasks. In the literature, high localization accuracy is achieved with the mainstream strongly supervised frameworks. However, such methods require object-level annotations and are unable to detect objects of unknown categories. Weakly supervised methods face similar difficulties. In this paper, a self-paced learning framework is proposed to achieve accurate object localization on the rank list returned by instance search. The proposed framework mines the target instance gradually from the queries and their corresponding top-ranked search results. Since a common instance is shared between the query and the images in the rank list, the target visual instance can be accurately localized even without knowing what the object category is. In addition to performing localization on instance search, the issue of few-shot object detection is also addressed under the same framework. Superior performance over state-of-the-art methods is observed on both tasks.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Analysis of Qualitative Results}

Some qualitative results are shown in Figure \ref{fig:more-examples}, our framework provides accurate box-level and pixel-level instance localization with no category restriction. However, there are still some issues that are remained to be addressed: (1) intra-class separation, (2) instance confusion. For the issue of intra-class separation, as shown in the last row of Figure \ref{fig:more-examples}, some similar false positives are also detected. This is caused by the lack of intra-class discrimination of features. For the issue of instance confusion, which is referred to the fact that when the target instance is too small or not significant enough, the features pooled from the query boxes are dominated by the features of other instances. The third image in last row in Figure \ref{fig:more-examples} is an example of the issue of instance confusion. The query is supposed to be Mario, but the extracted query features are dominated by the car, resulting in the false detection of the car instead of Mario in the reference image.
